Inductive Graph Embeddings through Locality Encodings

Learning embeddings from large-scale networks is an open challenge. Despite the overwhelming number of existing methods, is is unclear how to exploit network structure in a way that generalizes easily to unseen nodes, edges or graphs. In this work, we look at the problem of finding inductive network embeddings in large networks without domain-dependent node/edge attributes. We propose to use a set of basic predefined local encodings as the basis of a learning algorithm. In particular, we consider the degree frequencies at different distances from a node, which can be computed efficiently for relatively short distances and a large number of nodes. Interestingly, the resulting embeddings generalize well across unseen or distant regions in the network, both in unsupervised settings, when combined with language model learning, as well as in supervised tasks, when used as additional features in a neural network. Despite its simplicity, this method achieves state-of-the-art performance in tasks such as role detection, link prediction and node classification, and represents an inductive network embedding method directly applicable to large unattributed networks.

==> Sections/Experiments/classification.tex <==
In this section, we evaluate how IGEL is able capture structural attributes that generalize to unseen graphs from the same domain. 
%One of the key features of IGEL is that it is meant to capture structural attributes that generalize to unseen graphs from the same domain. To study if this is the case, we 
For that, we consider an inductive multi-label node classification task, in which we explore the performance of IGEL with or without pre-training and fine-tuning. The objective is to predict $121$ different binary labels capturing protein functions in a series of Protein-to-Protein Interaction (PPI) graphs. Aside from the graph structures, every node has an additional set of attributes, allowing us to evaluate how the performance of IGEL differs in attributed networks.
In this case, we use the supervised setting with the objective of Equation~\eqref{eq:supervised}.
%train our embeddings and then on models using only structural features or the concatenation of both structural and attribute features as inputs to a neural network.

We use the supervised baselines proposed by GraphSAGE~\cite{DBLP:journals/corr/HamiltonYL17-GraphSAGE} and LCGL~\cite{DBLP:journals/corr/abs-1808-03965-LGCL}, and further compare with a fully supervised version of GraphSAGE~\cite{velikovi2017graph-GAT}. We perform randomized grid search to identify the best possible set of parameters for an MLP containing IGEL and (optionally) feature inputs.

We analyze both encoding distances $\alpha \in \{1, 2\}$, with other IGEL hyper-parameters being fixed after a small greedy search based on the best configurations in the link prediction experiments. For the MLP model, we perform a greedy architecture search, including the number of hidden units, activation functions and depth. Our results show scores averaged over five different seeded runs with the same configuration, as obtained from the parameter search. We run each experiment on a machine with 8 cores, 16GB of memory and a single GPU with 8GB of device memory. 

\begin{table}[!h]
\centering
\caption{Micro-F1 scores for the multilabel classication task on the PPI graphs. IGEL combined with node features used as input for an MLP outperforms LGCL and supervised GraphSAGE both with and without sampling.}

\begin{tabular}{@{}llr@{}}
\toprule
\multicolumn{2}{l}{\textbf{Method}}             & \multicolumn{1}{l}{\textbf{PPI}} \\ \midrule
Random\textsuperscript{$\ddagger$}         &               & 0.396                            \\
Only Features (MLP, ours)                  &               & 0.558                            \\ \midrule
GraphSAGE-GCN\textsuperscript{$\dagger$}  &               & 0.500                             \\
GraphSAGE-mean\textsuperscript{$\dagger$} &               & 0.598                             \\
GraphSAGE-LSTM\textsuperscript{$\dagger$} &               & 0.612                             \\
GraphSAGE-pool\textsuperscript{$\dagger$} &               & 0.600                             \\ \midrule
GraphSAGE (no sampling)\textsuperscript{$\ddagger$} &     & 0.768                   \\
LGCL\textsuperscript{*}                   &               & 0.772                   \\ \midrule
\multirow{2}{*}{IGEL ($\alpha = 1$)}       & Graph Only    & 0.736                              \\
                                          & Graph + Feats & \textbf{0.850}                            \\ \midrule
\multirow{2}{*}{IGEL ($\alpha = 2$)}       & Graph Only    & 0.506                            \\
                                          & Graph + Feats & 0.741                            \\ \midrule
\end{tabular}
\caption*{\scriptsize \textsuperscript{} Results as reported by $\dagger$: \cite{DBLP:journals/corr/HamiltonYL17-GraphSAGE} $\ddagger$: \cite{velikovi2017graph-GAT} $*$: \cite{DBLP:journals/corr/abs-1808-03965-LGCL}}
\label{tab:PPIResults}
\end{table}

\autoref{tab:PPIResults} shows the classification results in terms of micro-averaged F1 score. 
Our model using structural embeddings and node features significantly outperforms both LGCL and every GraphSAGE instantiation with $\alpha = 1$. In this case, we find that a higher value of $\alpha = 2$ produces worse results than $\alpha=1$, which we attribute to overfitting. We believe that using regularization would help further improve these results. For reproducibility, we note that the best performing configuration is found with $\alpha = 2$ on $d = 256$ length embedding vectors, concatenated with node features as the input layer for 1000 epochs in a 3-layer MLP using ELU activations with a learning rate of 0.005. Additionally, we apply 100 epoch patience for early stopping monitoring the F1 score on the validation set.
%This result opens the door to the application or design of regularization techniques in the structural setting. 

Remarkably, we note that a model trained using only graph structural features at $\alpha = 1$ is able to outperform every GraphSAGE configuration that uses sampling. This highlights the strong predictive power of structural features alone, which is often disregarded when node or edges attributes are available.

%can be particularly strong in certain tasks such as this one.


==> Sections/Experiments/link_prediction.tex <==
We now evaluate IGEL on the task of predicting whether an edge exists between two given nodes.
To generate training data, we follow the methodology proposed in~\cite{DBLP:journals/corr/GroverL16-node2vec}, which allows us to compare with previous transductive algorithms.
%To perform the task and fairly evaluate our results against previous transductive models, we follow the methodology proposed for node2vec~\cite{DBLP:journals/corr/GroverL16-node2vec}. 
In particular, for a given graph, we generate negative examples (non-existing edges) by sampling random pairs of nodes that are not connected in the original graph. Positive examples (existing edges) are obtained by removing half of the edges while keeping the mutilated graph after the edge removals connected\footnote{The constraint of keeping the graph connected is only required to compare with transductive methods and not necessary for IGEL.}. Both sets of node pairs are chosen to have the same cardinality.

The mutilated graph is used to train the IGEL embeddings using the unsupervised objective of Equation~\eqref{eq:negsamp}. Once the weight matrix~$\mathbf{W}$ has been learned, we formulate a classification task, to classify pairs of nodes according to the labels described before.%distinguish existing edges in the mutilated graph from random node pairs.

For this final step, we use a logistic regression classifier with features corresponding to the Hadamard (element-wise) product of the embedding vectors of the nodes at each end of the predicted edge. This is the best combination of features reported in~\cite{DBLP:journals/corr/GroverL16-node2vec}. Note that this setting can be seen as a special case of our Equation~\eqref{eq:supervised} with $M=2$ and the deep architecture being replaced by a single layer of additional weights.

We optimize all hyper-parameters described in~\autoref{tab:UnsupervisedIGELParams}, together with the encoding distance, using grid search. Our experimental setting involves link prediction on in a social media setting in the Facebook ego-network graph, and a citation network on arXiv capturing collaboration between scientists.
We observe that the performance only depends strongly in two parameters: the encoding distance $\alpha$ and, to a lesser extent, the number of negative samples $z$. In general, we observe a diminishing returns effect, e.g., for $\alpha=3$ the performance is comparable to that of using $\alpha = 2$ while taking an order of magnitude more time. In Section~\ref{sec:Scalability} we evaluate empirically the impact of $\alpha$ in the complexity of the algorithm.


%To select our hyperparameters, we run a greedy search over the hyperparameter space varying encoding distances, vector lengths, number of epochs, window sizes and negative sample sizes. 
%using edges removed when sampling the original graph as the positive instances.
%not an inherent limitation of our model, as it could inductively learn to predict links between previously disconnected components. However, in order to fairly compare with existing methods, we leave the task of inductive link prediction over unattributed as future work.

%Previous transductive approaches need this, as otherwise the embeddings of nodes contained in disconnected components would learn distinct representations. 

%The connected graph that remains after sampling 50\% of the edges is then used to train network embeddings in an unsupervised way. On the learned embeddings, we train a logistic regression classifier to distinguish existing edges from random node pairs, using edges removed when sampling the original graph as the positive instances.
\begin{table}[H]
\centering
\caption{Area Under the ROC Curve (AUC) results for the Facebook and AstroPhysics arXiv graphs. IGEL outperforms transductive methods, only using local degree structure. Hyper-parameters are optimized using grid search in IGEL, and transductive methods are the best ones reported in~\cite{DBLP:journals/corr/GroverL16-node2vec}.}
\begin{tabular}{@{}lrr@{}}
\toprule
\textbf{Method}                                                                     & \textbf{Facebook}          & \textbf{arXiv}           \\ \midrule
DeepWalk \cite{DBLP:journals/corr/PerozziAS14-deepwalk} & 0.968            & 0.934          \\
LINE \cite{DBLP:journals/corr/TangQWZYM15-LINE}         & 0.949            & 0.890          \\
node2vec \cite{DBLP:journals/corr/GroverL16-node2vec}   & 0.968            & 0.937          \\ \midrule
IGEL                                                     & \textbf{0.976}   & \textbf{0.984}  \\\bottomrule
\end{tabular}
\label{tab:LinkPredictionAUROCResults}
\end{table}

\autoref{tab:LinkPredictionAUROCResults} shows the best performing configuration on a series of five independent experiments. The best performing configuration on the Facebook graph features $\alpha = 2$, learning $d = 256$ component vectors with $e = 10$ walks per node, each of length $s = 150$ and $p = 8$ negative samples per positive for the unsupervised negative sampling. Respectively on arXiv, we find the best configuration at $\alpha = 2$, $d = 256$, $e = 2$, $s = 100$ and $p = 9$. Finally, we note that we run each experiment on a machine with 8 cores, 16GB of memory and a single GPU with 8GB of memory. 

Compared to previous transductive approaches, which represent every individual node independently, our method represents nodes in terms of the aggregated representations of structural features within their neighbourhoods, which can lead to the same representation shared by different nodes. Despite this, IGEL outperforms previous methods such as DeepWalk, LINE and node2vec, that have access to the whole graph when learning node representations.

%in contrast, represents nodes only in terms of the aggregated representations of structural features within their neighbourhoods, which can mean that several nodes can share a single representation. Despite this, IGEL outperforms previous methods such as DeepWalk, LINE and node2vec that have access to the whole graph when learning node representations. 
%As a final note for the reader, we consistently find that configurations with $\alpha = 2$ consistently outperforms $\alpha = 1$. This is consistent with the intuition that larger encoding distances capture larger structural attributes, in a sense building a latent space analogous to that of non-neural methods such as common neighbour algorithms.



==> Sections/Experiments/overview.tex <==
Up to this point we have presented IGEL, a network embedding method that aims to be \textit{general}, \textit{inductive}, \textit{scalable} and that \textit{can be combined with deep neural methods}. In this section, we seek to demonstrate those properties of IGEL, formalizing in the following experimental hypotheses:

\begin{enumerate}
    \item \textit{Generality and Scalability.} The method, with varying hyper-parameters, should be capable of representing structural aspects in small and large graphs alike.
    \item \textit{Inductivity.} The method should learn representations from graphs seen during training that are applicable to unseen graphs in the same problem domain.
    \item \textit{Scalability and Compatibility with Deep Approaches.} The method should improve the performance of existing deep neural methods when used in conjunction with them without prohibitively impacting scalability.
\end{enumerate}

In the sub-sections that follow, we present a series of experiments tackling each of these experimental hypotheses and their results, using the graphs described in \autoref{tab:GraphsOverview}.  

\begin{table}[!h]
\centering
\caption{Overview of the graphs used in the experiments.}
\begin{tabular}{@{}lrrr@{}}
\toprule
                                                             & ~\textbf{\# Nodes} & ~\textbf{\# Edges}  & ~\textbf{Avg. Clust. Coeff.} \\ \midrule
Les Miserables (cloned)                                      & 154       & 509     & 0.73 \\
Sister Cities~\cite{AKaltenbrunner13-SisterCities}           & 11~618    & 15~225  & 0.11 \\
Facebook~\cite{snapnets}                                     & 4~039     & 88~234  & 0.52 \\
ArXiv AstroPhysics~\cite{snapnets}                           & 18~772    & 198~050 & 0.32 \\
PPI (train)~\cite{DBLP:journals/corr/HamiltonYL17-GraphSAGE} & 44~906    & 613~184 & 0.12 \\ \bottomrule
\end{tabular}
\label{tab:GraphsOverview}
\end{table}



==> Sections/Experiments/study.tex <==
We first evaluate IGEL in the unsupervised setting using networks that are amenable for visual analysis. We focus on analyzing how the encoding distance parameter~$\alpha$ influences the learned representations.
%For this, we consider two networks, the popular Les Misérables network~\cite{miserables} and the Sister Cities network~\cite{AKaltenbrunner13-SisterCities}.
%and analyze 
%To do so, we look at how the encoding distance hyper-parameter behaves, as it defines most of how IGEL functions. Our study focuses on raw representation learned on two graphs. 
%We start by studying how the encoding distance impacts the representation in a small graph to illustrate how IGEL works. We do so by training unsupervised IGEL embeddings on a small graph with encoding distances ranging from 1 to 4. On those embeddings, we learn k-means clustering models and discuss the arising patterns and how they relate to the structural encodings.
%We first analyze 

\emph{Les Misérables Network}--- 
In this task, we consider a variation of the original Les Misérables network~\cite{miserables} in which two identical copies of the network are connected by an edge between two nodes from each copy selected randomly, as shown in~\autoref{fig:MiserablesClustering}. This allows us to analyze how the IGEL embeddings can capture structural similarity from distant areas of the graph.

We first use IGEL to learn feature representations for every node, and subsequently cluster the obtained embeddings. For a complete description of the experiment and parameter settings, see Appendix~\ref{app:case}.

\autoref{fig:MiserablesClustering} shows the composite network with nodes colored based on their clusters. For $\alpha = 1$, the local encodings only consider direct neighbours.
In this case, the resulting embeddings capture the standard notion of community or homophily, i.e., nodes with the same color are densely connected between each other and weakly connected to the rest. Furthermore, the embeddings 
corresponding to nodes within the two copies of each community also appear clustered together, although some nodes are not directly connected. This shows that IGEL embeddings can capture 
structural similarity, not only locally, but also from distant nodes in the graph.
\begin{figure}[!b]
    \centering
    \begin{subfigure}{0.49\linewidth}
        \centering
         \includesvg[width=\linewidth]{MiserablesClonedCaseStudy/MiserablesCloned-D1-K6-HarmCloseness.svg}
        \caption{Node clusters at encoding distance $\alpha = 1$.}
    \end{subfigure}
    \begin{subfigure}{0.49\linewidth}
        \centering
        \includesvg[width=\linewidth]{MiserablesClonedCaseStudy/MiserablesCloned-D2-K6-HarmCloseness.svg}
        \caption{Node clusters at encoding distance $\alpha = 2$.}
    \end{subfigure}
    %\caption{Clustering results produced by running k-means clustering  (with $k = 6$) over the IGEL embeddings trained with an encoding distance of $\alpha = 1$ (left) or $\alpha = 2$ (right). Node sizes correspond to their harmonic closeness centrality score. }
    \caption{Visualization of the embeddings in the (cloned) Les Mis\'erables network: node colors reflect the clustering of the embeddings obtained for two different encoding distances, $\alpha = 1$ (left) or $\alpha = 2$ (right).
    In addition to capture community structure, the IGEL embeddings also generalize structurally similar nodes between distant regions.
    Node sizes correspond to their harmonic closeness centrality score. }
    \label{fig:MiserablesClustering}
\end{figure}

%Our input is the graph of character co-occurrences in Victor Hugo's Les Misérables. We use a cloned version of the graph in which all nodes and edges in the original graph are duplicated as two independent disconnected components. We then connect the two disconnected components using a single edge between two randomly chosen nodes, and use the resulting graph to show that the structural aspects are preserved across both copies of the graph.

%Since our problem is a graph problem, we borrow from graph community detection techniques and metrics. The quality of the clusters detected in a graph is by often measured by means of the modularity score~\cite{PhysRevE.69.026113-modularity}. A high modularity means that the groups found in graph contain nodes linking with other members of the same group more often that you would expect by random chance. For every encoding distance, we identify the number of k-means clusters that maximise the modularity score, as shown in \autoref{fig:MiserablesModularity}. It is those node groupings that we show to discuss how the model functions\footnote{We also tried to identify the most informative number of clusters using the elbow method but no clear candidates emerged, as shown in \autoref{fig:MiserablesElbowPlots}}. As a structural method, IGEL is meant to capture local structures and how they interact with one another, as shown in \autoref{fig:MiserablesClustering}.

Larger encoding distances allow IGEL to capture relationships on larger portions of the graph. For $\alpha = 2$, shown in~\autoref{fig:MiserablesClustering}(b),
the embeddings are clustered in two major groups, separating frequently visited nodes---with higher degrees and closeness centrality, and hence more commonly appearing in the sampling process---from connecting bridges or edges.

%Conversely, a smaller encoding distance allows IGEL to detect communities of nodes displaying similar connectivity (i.e similar degrees), as seen in the dark green cluster when $\alpha = 1$, which contains an otherwise distant node. 
%The clusterings are mirrored on both graphs, except for the nodes joined by the the bridge. On a larger graph, only structural, local aspects will be preserved, as otherwise prohibitively expensive encoding distances may be needed to represent global relationships. With this hypothesis, we would expect that centrality measures such as closeness will be harder to capture as a graph grows larger. We explore this idea in the following section. 

%translates into separating frequently visited nodes---with higher degrees and closeness centrality, and hence more commonly appearing in the sampling process---from connecting bridges or edges. Conversely, a smaller encoding distance allows IGEL to detect communities of nodes displaying similar connectivity (i.e similar degrees), as seen in the dark green cluster when $\alpha = 1$, which contains an otherwise distant node. The clusterings are mirrored on both graphs, except for the nodes joined by the the bridge. On a larger graph, only structural, local aspects will be preserved, as otherwise prohibitively expensive encoding distances may be needed to represent global relationships. With this hypothesis, we would expect that centrality measures such as closeness will be harder to capture as a graph grows larger. We explore this idea in the following section. 

%\subsubsection{}
\emph{Sister Cities Network}--- 
We now illustrate how IGEL can be used for knowledge discovery using a larger network: the network of Sister Cities~\cite{AKaltenbrunner13-SisterCities}, a graph mined from Wikipedia where nodes correspond to cities and links to partnerships.
We follow a similar approach as before and train IGEL embeddings for each node.
We then perform a clustering analysis of the embeddings. Appendix~\ref{app:sister} shows the details of the setup.

%and study the relationship of the learned node embeddings with network centrality measures such as Degree or PageRank. Furthermore, we showcase how an unsupervised clustering captures real world patterns. 

%After gaining an intuition of how the model learns its representations, we focus on studying the ability of the model to capture semantic patterns in an unsupervised way. We apply IGEL on a graph of Sister Cities mined from Wikipedia~\cite{AKaltenbrunner13-SisterCities} and study the relationship of the learned node embeddings with network centrality measures such as Degree or PageRank. Furthermore, we showcase how an unsupervised clustering captures real world patterns. 

%We ought to understand how the representation relates to other graph metrics such as centrality measures. One possible way of carrying such study is to develop a predictive model that estimates measures such as PageRank or Degree centrality from the embedding vectors. However, this would not only describe the representation learned by the IGEL model, but rather involve two models, one of which is supervised, and it would not be straightforward to identify whether the relation with the graph measures come from IGEL or the learned model. To avoid aforementioned interpretability problem, we opt for a different approach. 

\begin{figure}[!t]
    \centering
    \includesvg[width=\linewidth]{SisterCitiesCaseStudy/MercatorSisterCitiesD4K6CapitalsLBG-LargerDots.svg}
    \caption{Geo-plot of the learned clusters on the Sister Cities dataset, filtering only cities that are capitals. Each point is a city, with a radius proportional to its degree, and colored by the group assigned by the clustering model. To learn the clusters, we use an IGEL encoding distance $\alpha = 4$ and rum KMeans with $k = 6$. }
    \label{fig:SisterCities}
\end{figure}
%Beyond simple correlation statistics, we want to understand if the model captures high level aspects of the graph. To do so, 

The obtained clusterings allows us to identify interpretable roles for the nodes, for example, cities that are country capitals. To quantitatively test this, we use an external labeled dataset that assigns a total of $179$ nodes as country capitals, and then evaluate IGEL as a binary classifier by treating the nodes that belong to the cluster containing the highest number of capital cities as positive, and the rest of the nodes as negative.

\autoref{fig:SisterCities} shows a geo-plot with label colors corresponding to a subset of $872$ capital cities. Remarkably, this cluster composed of IGEL embeddings consistently outperforms heuristic methods by capturing up to 28\% more country capitals, as measured by F1-score (see~\autoref{tab:SisterCitiesF1Scores} in the Appendix for details).
From these results, we can conclude that IGEL is also effective discovering non-trivial embeddings that are interpretable.

%baseline with a heuristic approach based on node degree and PageRank score. We rank the nodes by either metric and take as many nodes as there are in the positive cluster. We then compute F1-scores for the cluster, degree and PageRank approaches, as shown in . 

%Then, using a labeled dataset that identifies 179 nodes as country capitals, we evaluate the model as a binary classifier as follows. We treat the cluster containing the most capital cities as the positive indicator, in which all nodes belonging to it are classified as capitals. We consider that nodes falling in any other cluster are assigned to the negative class. In this way, our unsupervised clustering model effectively becomes a one-vs-all classifier.

%To compare the clustering model, we set a baseline with a heuristic approach based on node degree and PageRank score. We rank the nodes by either metric and take as many nodes as there are in the positive cluster. We then compute F1-scores for the cluster, degree and PageRank approaches, as shown in \autoref{tab:SisterCitiesF1Scores}. 





==> Sections/abstract.tex <==
%% Text of abstract
%15--250 words.compact 
Learning embeddings from large-scale networks is an open challenge.
Despite the overwhelming number of existing methods, is is unclear
how to exploit network structure in a way that generalizes easily to unseen nodes, edges or graphs.
%Despite the overwhelming amount of existing algorithms, current methods exploit network structure in manners that do not easily generalize to unseen nodes, edges or graphs. 
%For example, although graph convolutional networks achieve impressive performance on complex inductive tasks, it is unclear to what extent they rely on the existence of node or edge attributes.
In this work, we look at the problem of finding inductive network embeddings in large networks without domain-dependent node/edge attributes. We propose to use a set of basic predefined local encodings as the basis of a learning algorithm.
In particular, we consider the degree frequencies at different distances from a node, %as ``prior'' local features, %This \emph{prior} features 
which can be computed efficiently for relatively short distances and a large number of nodes. 
Interestingly, the resulting embeddings generalize well across unseen or distant regions in the network, both in unsupervised settings, when combined with language model learning, as well as in supervised tasks, when used as additional features in a neural network.
%when such features are used in standard embedding techniques, as well as in predefined features in supervised tasks, they generalize well across unseen or distant regions in the network.%has a dramatic effect when combined with standard embedding techniques.
Despite its simplicity, this method achieves state-of-the-art performance in tasks such as role detection, link prediction and node classification, and represents an inductive network embedding method directly applicable to large unattributed networks.

==> Sections/conclusions.tex <==
In this work we have presented IGEL, a novel inductive network embedding method that compactly captures graph structures in a dense latent space. To the best of our knowledge, IGEL is the first inductive embedding algorithm explicitly designed for unattributed graphs that captures structural features without the need for node attributes. 

Our results show that IGEL is scalable and can compete with transductive approaches in tasks such as link prediction on unattributed graphs. Additionally, IGEL can inductively generalize to unseen graphs, outperforming models based on Graph Convolutional Networks in a multi-label classification setting. Our work also highlights future directions for research, namely, regarding the improvement of time and memory consumption, finding ways to capture global aspects of a graph that IGEL cannot represent, and managing the evolution of degree-based structural features in temporal graphs. 


==> Sections/experiments.tex <==
%In this section, we present a series of experiments to evaluate IGEL. First, we describe the experimental hypotheses that act as the rationale for our experiments. Then, we study community detection and network centrality estimation using IGEL on a small network. Afterwards, we evaluate the ability of our method to capture local relationships between nodes on link prediction tasks in medium-sized graphs. Finally, we apply IGEL to an inductive multilabel node classification task in a large collection of protein graphs. 

In this section, we evaluate IGEL in different tasks. We first analyze visually the type of structural properties captured by the method. Then, we evaluate the method in link prediction tasks for medium-sized graphs. Finally, we apply IGEL to an inductive multilabel node classification task in a large collection of protein graphs. For this analysis, we use the graphs described in \autoref{tab:GraphsOverview}.
\begin{table}[!t]
\centering
\caption{Overview of the graphs used in the experiments.}
\begin{tabular}{@{}lrrr@{}}
\toprule
                                                             & ~\textbf{\# Nodes} & ~\textbf{\# Edges}  & ~\textbf{Avg. Clust. Coeff.} \\ \midrule
Les Miserables (cloned)                                      & 154       & 509     & 0.73 \\
Sister Cities~\cite{AKaltenbrunner13-SisterCities}           & 11~618    & 15~225  & 0.11 \\
Facebook~\cite{snapnets}                                     & 4~039     & 88~234  & 0.52 \\
ArXiv AstroPhysics~\cite{snapnets}                           & 18~772    & 198~050 & 0.32 \\
PPI (train)~\cite{DBLP:journals/corr/HamiltonYL17-GraphSAGE} & 44~906    & 613~184 & 0.12 \\ \bottomrule
\end{tabular}
\label{tab:GraphsOverview}
\end{table}
%Up to this point we have presented IGEL, a network embedding method that aims to be \textit{general}, \textit{inductive}, \textit{scalable} and that \textit{can be combined with deep neural methods}. In this section, we seek to demonstrate those properties of IGEL, formalizing in the following experimental hypotheses:
The goal of this section is to evaluate experimentally the following hypothesis:
\begin{enumerate}
    \item \textit{Generality and scalability:} the method should be capable of representing structural aspects in small and large graphs alike. %, with varying hyper-parameters,
    \item \textit{Inductivity:} the method should learn representations from graphs seen during training that generalize to unseen graphs from the same domain.
    \item \textit{Scalability and compatibility with deep learning approaches:}
    the method should outperform or be competitive with existing deep neural methods when used in conjunction with them without incurring in too excessive additional costs.
\end{enumerate}
%In the sub-sections that follow, we present a series of experiments tackling each of these experimental hypotheses and their results, 

%\subsection{Experimental Setting}
%\input{Sections/Experiments/overview}

\subsection{Unsupervised Setting}
\input{Sections/Experiments/study}

\subsection{Link Prediction}
\input{Sections/Experiments/link_prediction}

\subsection{Node Classification}
\input{Sections/Experiments/classification}


==> Sections/igel.tex <==
In this section we describe IGEL in detail. We first provide an overview of the method and then drill down into the two steps that compose its high level algorithm. As IGEL embeddings can be trained in either supervised or unsupervised settings, we close the section with a formal description of the different objectives, paving the way for the experimental section of this work.

\subsection{Overview}

The main idea of IGEL is to represent local graph structures inductively by learning dense embeddings over a sparse space of structural attributes that appear in the surroundings of nodes in a graph. These dense embeddings can be learned in supervised or unsupervised ways, with the overall process encompasing two main steps. For a given graph $\mathcal{G} = \langle V, E \rangle$ composed of a set of vertices $V$ and edges $E$, representing a node requires:

\begin{enumerate}
  \item \textbf{Encoding.} The first step encodes local graph structures in the form of a sparse vector recording the frequencies of structural attributes found for every given node $n \in V$.
  \item \textbf{Embedding.} The sparse encoding is used as input to an embedding model, that transforms the input vector into a dense representation of the aggregated structural attributes.
\end{enumerate}

%We provide a detailed description of the two steps in the sub-sections that follow, as well as the optimization processes employed to train the embeddings.

\subsection{Encoding Local Graph Structures}
\label{sec:encoding}
%To represent a node, the first step of the algorithm consists in capturing graph structures that can suitably be embedded.
We capture the local structure by considering the neighbourhood of a node. %, the first step of the algorithm consists in capturing graph structures that can suitably be embedded.
 For a given node $n \in V$ and encoding distance $\alpha\in \mathbb{N}$, let $\mathcal{G}_{\alpha}(n)$ denote the sub-graph of $\mathcal{G}$ containing all nodes found at distance at most $\alpha$ from~$n$, and the edges connecting them. From the neighbourhood graph $\mathcal{G}_{\alpha}(n)$, we represent the structural features of node $n$ by considering the number of times a degree $d$ is found at distance $c$ in the graph $\mathcal{G}_\alpha(n)$, $c=0, \hdots, \alpha$.

In this way, the structural features can be understood as a succession of distance $c \in \mathbb{N}$ and degree $\delta \in \mathbb{N}$ tuples $(c, \delta)$ and their respective counts. Given the max-degree $\delta_\text{max}$ of $\mathcal{G}$, a sparse feature vector $\mathbf{x}_n \in \mathbb{R}^\ell$, with $\ell =~\delta_\text{max} \times \alpha$, can be constructed such that %$x_i^{(n)}$,
the $i$th component of $\mathbf{x}_n$, $i = c\delta_\text{max}  + \delta$, contains the number of times the tuple $(c, \delta)$ appears in $\mathcal{G}_\alpha(n)$. A visual representation of this encoding process is shown in \autoref{fig:GraphStructureEncoding}.

\begin{figure}[!t]
    \centering
    \includegraphics[width=0.65\linewidth]{Diagrams/GraphStructure.pdf}
    \caption{Encoding example. The dashed region denotes the corresponding neighbourhood of the green node $n$ for distance $\alpha = 2$. \textcolor{green!60!black}{Green nodes} are at distance \textcolor{green!60!black}{$0$}, \textcolor{blue!75!black}{blue nodes} at \textcolor{blue!75!black}{$1$} and \textcolor{red!80!black}{red nodes} at \textcolor{red!80!black}{$2$}. Numbers indicate the degrees within the induced graph. The structural representation for the green node is the following frequency mapping of distance-degree $(c, \delta)$ pairs: $\{
        \textcolor{green!60!black}{(0, 2): 1},
        \textcolor{blue!75!black}{(1, 2): 1},
        \textcolor{blue!75!black}{(1, 4): 1},
        \textcolor{red!80!black}{(2, 3): 2},
        \textcolor{red!80!black}{(2, 4): 1} 
    \}$, which translates into the sparse structural feature vector $\mathbf{x}_n$ shown at the bottom. 
    }
    \label{fig:GraphStructureEncoding}
\end{figure}

The proposed encoding can be further processed and normalized. In this work, we log-normalize each feature count $z$ as $\log_2(1 + z)$ and then normalize the transformed features to the $[0, 1]$ interval. Also, if during testing we need to compute the features for a new node with degree $\delta'>\delta_\text{max}$, we use the bin corresponding $\delta_\text{max}$ to store its frequency.

\subsection{Embedding of the Sparse Representations}

At this point, we can represent a node in terms of its immediate surroundings, but this representation is sparse and high dimensional. A simple way to transform the sparse structural features into a dense, lower dimensional, representation is through a linear transformation:
\begin{align}
    \mathbf{e}_n & =\mathbf{x}_n^\top \cdot \mathbf{W},
    \label{eq:SimpleModel}
\end{align}
where $\mathbf{e}_n$ is $d$-dimensional, and $\mathbf{W} \in \mathbb{R}^{\ell \times d}$ is a learnable matrix of parameters, $d\ll \ell$. Each row in $\mathbf{W}$ captures the vector representation of each single structural feature. Intuitively, this can be understood as a weighted average of the encoded structural features, representing the node in terms of its immediate surroundings. \autoref{fig:StructuralEmbedding} provides a visual overview. %for the reader.

\begin{figure}[!t]
    \centering
    \includegraphics[width=1.0\linewidth]{Diagrams/StructuralEmbedding.pdf}
    \caption{Structural embedding example. Shaded regions in $\mathbf{x}_n$ refer to the zero values in the sparse representation, which in turn represent unseen structures as seen in $\mathbf{W}$. The dense representation of node $n$ is $\mathbf{e}_n$, as seen in \autoref{eq:SimpleModel}. The final vector, represented in step $4$, is the linear combination of the structural feature matrix combined with the sparse feature vector, with each strip representing the value of the source structure in the embedding matrix and its width indicating the contribution to that particular component.}
    \label{fig:StructuralEmbedding}
\end{figure}

\subsection{Learning the Embeddings}

We now describe the learning procedure for the parameters $\mathbf{W}$ such that the general structural properties of the original encoding are preserved.
%, recall that the encoding function defined previously provides a representation of the structure surrounding any node in the graph in the form of a sparse vector. For any such sparse vector, an embedding model produces a dense representation in its forward pass, ideally preserving the general structural properties of the original encoding. 
Such properties to preserve are task-dependent: 
in exploratory network analysis, we aim to learn representations that capture general graph properties such as degree distributions, centrality measures, or structural similarities. In classification tasks, the objective is to identify attributes that are useful to discriminate between the classes, if the model can capture them. We now define the two optimization objectives considered by IGEL corresponding to both scenarios.

%Under this lens, the optimization task can be understood as either supervised or unsupervised. In the sections following, we further describe both approaches.

\subsubsection{Unsupervised Setting}

Our objective in the unsupervised setting is to capture the global network features in terms of the local structures surrounding every node. We formulate this problem similarly to skip-gram based methods~\cite{DBLP:journals/corr/GroverL16-node2vec,DBLP:journals/corr/PerozziAS14-deepwalk}, which optimize a likelihood function from sample data generated through random walks on the graph. In the following, we describe the two steps involved in learning the embeddings. 
%Unlike skip-gram methods that use each individual node in the samples, we consider the corresponding local encoding in the objective function.

%\vspace{.25cm}
\emph{Distributional Sampling through Random Walks}---
%Our sparse vectors explicitly capture the local information of each node and, importantly, they can also be computed for nodes that did not exist during training time. However, we are interested in learning dense representations that capture network information at the global level. 
%Our objective now becomes to capture the relationships of such structural properties for a given graph. Typically, such relationships can be learned using a sampling approach, which
Our sampling strategy generates sample paths over the graph, %~\cite{DBLP:journals/corr/PerozziAS14-deepwalk}
selecting the next node uniformly from the neighbours of the current node.
%the Markov chain with state space $V$ and transition matrix $P(u,v)=1/\texttt{deg}(u)$, if $(u,v)\in E$, and $0$ otherwise~\cite{DBLP:journals/corr/PerozziAS14-deepwalk}. 
\autoref{fig:GraphStructureSampling} illustrates a possible random walk of length 9 in the same graph of~\autoref{fig:GraphStructureEncoding}. Each node contains the time-step(s) when it was visited during the random walk.

This step is similar to existing sample-based transductive methods, such as DeepWalk~\cite{DBLP:journals/corr/PerozziAS14-deepwalk}. In contrast to other methods such as node2vec~\cite{DBLP:journals/corr/GroverL16-node2vec}, our method uses unbiased random walks, and does not require tuning of the probabilities of in-out and return paths when sampling each graph. Additionally, our approach does not require any previous computation of a structural meta-graph, as proposed by struct2vec~\cite{DBLP:journals/corr/FigueiredoRS17-struct2vec}. Instead, we perform $w$ random walks of length $s$ starting from each node in the network.
\begin{figure}[!t]
    \centering
    \includegraphics[width=0.65\linewidth]{Diagrams/GraphRandomWalk.pdf}
    \caption{Example of random walk. Nodes contain the time-step when they were visited. The context of nodes seen besides a target node across the walk serves to learn the representations given by the approach shown in \autoref{fig:GraphStructureEncoding}.}
    \label{fig:GraphStructureSampling}
\end{figure}

As we randomly sample the structure of the graph, we produce sequences of traversed nodes.
These sequences are used in the optimization objective we describe next.
%In the next section we describe the unsupervised approach under which we use those co-occurrences to train the embeddings.

%\vspace{.25cm}
\emph{Negative Sampling Optimization Objective}---
Given a random walk $\omega$, defined as a sequence of nodes of length $s$, we define the context $\mathcal{C}(n, \omega)$ associated to the occurrence of a node $n$ in $\omega$ as the the sub-sequence in $\omega$ containing the nodes that appear close to $n$, including repetitions. Closeness is determined by the hyper-parameter $p$, the size of the positive context window, i.e., the context contains all nodes that appear at most $p$ steps before/after the node within $\omega$.

Similarly to DeepWalk or node2vec, we define a skip-gram negative sampling objective that learns to identify nodes appearing in similar contexts within the random walks. Given a node $n_t \in V$ in random walk $\omega$, our task is to learn embeddings that 
assign high probability for nodes $n_o\in V$ appearing in the context $\mathcal{C}(n_t, \omega)$, and lower probability for nodes not appearing in the context. As we focus on the learned representation capturing these symmetric relationships, the probability of $n_o$ being in $\mathcal{C}(n_t, \omega)$ is given by:
\begin{align}
 p\left(n_o \in \mathcal{C}(n_t, \omega)\right) &= \sigma(\mathbf{e}^\top_{n_t} \cdot \mathbf{e}_{n_o}),
\end{align}
where $\sigma(\cdot)$ is the logistic function. 
\begin{table}[!t]
\centering
\caption{Hyper-Parameters used in unsupervised tasks.}
\begin{tabular}{@{}ll@{}}
\toprule
\textbf{Hyper-Parameter}    & \textbf{Description}                 \\ \midrule
$w \in \mathbb{N}$ & Number of random walks per node       \\ 
$s \in \mathbb{N}$ & Number of steps in the Random Walks  \\ 
$z \in \mathbb{N}$ & Proportion of negative examples      \\ 
$p \in \mathbb{N}$ & Positive samples context window size \\ 
\midrule \end{tabular}
\label{tab:UnsupervisedIGELParams}
\end{table}

The global objective function is the following negative sampling log-likelihood to be maximised. For each random walk and each node in the random walk, we sum the term corresponding to the positive cases for structures found in the context, and the expectation over $z$ negative, randomly sampled, structures:
\begin{align}\label{eq:negsamp} %\text{arg}\max_{\mathbf{W}} \left(
  \mathcal{L}_{\text{u}}(\mathbf{W})&= \sum^{w}_{j=1} \sum_{
  \substack{n_t \in \omega_j,\\
  n_o \in \mathcal{C}(n_t, \omega_j)}}  \Bigg[\log \sigma(\mathbf{e}_{n_t}^\top \cdot \mathbf{e}_{n_o}) + \sum^z_{i=1}  \mathbb{E}_{{n_i} \sim P_n(V)} \Big[\log \sigma(-\mathbf{e}_{n_t}^\top \cdot \mathbf{e}_{n_i})\Big]\Bigg],
\end{align}
where $P_n(V)$ is the noise distribution from which the $z$ negative samples are drawn.
We maximize~\eqref{eq:negsamp} through gradient ascent. \autoref{tab:UnsupervisedIGELParams} summarizes the hyper-parameters in the unsupervised setting.

\subsubsection{Supervised Setting}

Besides its direct usage as an inductive node embedding method, IGEL can also be used as a node embedding layer in a deep neural network. In particular, the embedding of Eq.~\eqref{eq:SimpleModel} can be fed into a downstream model as additional input features for a multilayer perceptron (MLP) or a graph neural network (GNN). 
In this case, the weight matrix $\mathbf{W}$ is jointly learned with the rest of the model parameters $\boldsymbol{\Theta}$. Instead of capturing global structural properties through random walks as before, the model in the supervised setting captures salient structural features that have predictive power in a particular task.

\autoref{fig:GraphSupervisedLearning} illustrates the general model for a standard node classification task, in which the IGEL embeddings are used in combination with possibly additional node attributes $\mathbf{F}_n$ to generate a final output $\hat{y}$ that is used to predict the node class label.

% in a supervised learning setting. 

%This means that IGEL embeddings can serve as another input feature for a multilayer perceptron (MLP) or graph neural network (GNN) in a supervised learning setting. 

%In a supervised environment, the forward IGEL pass will remain the same, but its output embeddings will be fed into a downstream model that is then trained to perform node or edge level inference. 

%We consider node classification as an example task. In this case, 

%to identify structural attributes that indicate the presence of one class or the other.
%that is then trained to perform node or edge level inference. 

\begin{figure}[!t]
    \centering
    \includegraphics[width=0.7\linewidth]{Diagrams/IGELSupervised.pdf}
    \caption{An example of IGEL applied in a supervised setting.
    The node embedding $\mathbf{e}_n$ provides a structural representation that can optionally be combined with additional node or edge features as an input to a deep learning model which outputs $\tilde{y}$.
    The weight matrix $\mathbf{W}$ is jointly learned with the rest of the parameters $\boldsymbol{\Theta}$.
    See text for details.}
    \label{fig:GraphSupervisedLearning}
\end{figure}

Using IGEL as a feature layer additionally allows for pre-training and fine-tuning when data is not sufficiently available. This is similar to natural language domains, where language models are first trained on large corpora and then retrained for specific tasks at hand.
Analogously, the IGEL layer can be learned first in the unsupervised manner described in the previous section, and subsequently refined to a specific inference task. 

Without loss of generality, we focus on multi-label classification without pre-training. For $M$ independent labels, the task is to minimise the binary cross-entropy of the predicted labels associated to nodes:
%\begin{align}
%- \frac{1}{M} \sum_{i=1}^M y_n^i \log\Big(\sigma(\hat{y}_n^i)\Big)
%                         + (1-y_n^i) \log\Big(\frac{\sigma(\hat{y}_n^i)}{e^{\hat{y}_n^i}}\Big)
%\end{align}
\begin{align}\label{eq:supervised}
\mathcal{L}_{\text{s}}(\mathbf{W},\boldsymbol{\Theta}) &= - \sum_{n\in V}\sum_{i=1}^M \Big[ y_n^i
\log
\sigma(\hat{y}_n^i) +
(1-y_n^i) \log\left(1-\sigma(\hat{y}_n^i)\right)\Big],
\end{align}
%Where $y_n^i$ is the expected value in the ground truth for the $i$-th class assigned to node $n$ and $\hat{y}_n$ are the $M$ actual class activations produced by a model $\phi$ when input with the output from the IGEL embedding function on $n$ and node attributes $\mathbf{F}_n$ if available:
where $y_n^i$ is one if $i$ is the true class label of node $n$, and zero otherwise, and $\hat{y}_n^i$ is the network output corresponding to the class with label $i$.
%\begin{align}
%\hat{y}_n = \phi\Big(\mathbf{e}_n \oplus \mathbf{F}_n\Big)
%\end{align}

\subsection{Computational Complexity}

%We now describe the computational complexity of IGEL in relation to the other methods. We describe the time and parameter complexities of other methods as described by \cite{GOYAL201878, DBLP:journals/corr/abs-1901-00596}. We express cost with respect to the input, namely, the graph being encoded. Time complexity is expressed in terms of computation steps during the training process, while parameter complexity refers to the number of learnable parameters that are defined by each model. For example, a time complexity $\mathcal{O}(|V|)$ means that the time cost of the training process scales linearly with regards to the number of nodes in the graph. We note that certain parameters such as the number of random walks or their length in sampling-based methods appear as a constant, which we do not include in our analysis. 
We now describe the computational complexity of IGEL in relation to other embedding methods. Time and parameter complexities of other methods is described as in~\cite{GOYAL201878, DBLP:journals/corr/abs-1901-00596}. %We express cost with respect to the input, namely, the graph being encoded. 
We differentiate time complexity, expressed in terms of computational steps given an input graph, and parameter complexity, which refers to the number of learnable parameters corresponding to a particular model. %For example, a time complexity $\mathcal{O}(|V|)$ means that the time cost of the training process scales linearly with regards to the number of nodes in the graph. 
We note that certain parameters such as the number of random walks or their length in sampling-based methods appear as a constant, which we do not include in our analysis. 

%To illustrate the analysis, we describe our derivation of both complexities for IGEL.
%Due to its training process, whether supervised or unsupervised, we expect to update the representation of every node a constant number of times, hence $\mathcal{O}(|V|)$.
%In IGEL, we expect to update the representation of every node a constant number of times, hence the time complexity scales linearly as $\mathcal{O}(|V|)$.
We first consider the parameter complexity. Let $\gamma$ be the number of bins required to encode the local degree-based representation, which we set to the maximum degree $\delta_{\text{max}}$ in this work\footnote{For highly skewed degree distributions, the original algorithm can be modified to require less parameters $\gamma \ll \delta_{\text{max}}$ by using log-sized bins or exploiting the sparsity of the feature vectors.}. Since each embedding vector has dimension~$d$ and we have $\gamma$ bins for each encoding distance, the number of parameters scales as $\mathcal{O}(\alpha\times\gamma\times d)=\mathcal{O}(\ell\times d)$.

On the other hand, the time complexity involves two main steps: a pre-processing step that computes the encoding of the local representations, and the computations required at each optimization step. The encoding step requires to visit all nodes at distance $\alpha$ from each node $n$, and repeat that for each node in the graph, therefore the time complexity is exponential in~$\alpha$, $\mathcal{O}(|V|\times \delta_{\text{max}}^{\alpha})$. 
Once the local representations are computed, however, the optimizations step can be done efficiently, involving only a product that grows linearly with the number of parameters, or a forward-pass in a neural network.

%Every update means at most propagating the error signals to
%$\gamma$ bins at a maximum encoding distance $\alpha$, i.e., to~$\psi^\alpha$ updates per node, leading to a 
%The parameter complexity follows a similar line of reasoning. Let the maximum degree be $m$ and $\alpha$ the encoding distance, we have a $d$-dimensional embedding vector for each structural representation pair. Thus, an IGEL model ought to have $\mathcal{O}(\alpha m d)$ parameters\footnote{Note that in case of skewed degree distributions, the algorithm could be easily modified to use a lower value of $d$ than the max degree, encoding all higher-degree neighbours into the same max bin $d$.}. 

\autoref{tab:ComplexityComparison} compares the time and parameter complexities of several models. Transductive models such as DeepWalk, node2vec or struct2vec scale linearly with respect to the number of nodes, both in terms of time and parameters. Inductive methods based on  graph convolutions incur in higher training costs, as signals have to be propagated across the whole set of nodes and edges. Their parameter complexity, however, is not directly dependent on either, and is instead a function of the number of input features. Sampling-based methods such as GraphSAGE reduce the time complexity cost by ensuring that a fixed number of sampled nodes are used during training and inference.

We note that IGEL lies at the crossroads of the previous methods. Its time complexity depends on both the number of nodes and the size of their surrounding neighbourhoods, similar to sampling-based GCNs. However, IGEL lacks the fixed bounds in the number of operations that is guaranteed by sampling a constant number of nodes at a time. Due to this fact, we expect IGEL's performance to degrade on denser graphs with neighbourhoods containing a wider range of different degrees among their nodes. Finally, IGEL's parameter complexity is closer to transductive methods, with a bound given by the maximum degree in the graph.

\begin{table}[!h]
\centering
\caption{A comparison of graph representation methods in terms of their average parameter and time complexities. The parameters $\alpha$ stands for IGEL's encoding distance, $r$ is the sampling factor for sampling GCNs, $\rho$ is the convolutional distance in GCNs, $\delta_{\text{max}}$ is the maximum degree and $d$ is either the size of the embedding vectors or the number of features, depending on the method.}
\begin{tabular}{@{}lrr@{}}
\toprule
\textbf{Name}                    & \textbf{Time Complexity}           & \textbf{Parameter Complexity} \\ \midrule
\textit{DeepWalk, node2vec}      & $\mathcal{O}(|V|)$                 & $\mathcal{O}(|V|d)$           \\
\textit{struct2vec\textsuperscript{*}} & $\mathcal{O}({|V|} \log |V|)$      & $\mathcal{O}(|V|d)$      \\
\textit{GCN}                     & $\mathcal{O}(\rho |V| |E|)$        & $\mathcal{O}(\rho d^2)$       \\
\textit{GraphSAGE}               & $\mathcal{O}(r^\rho |V|)$          & $\mathcal{O}(\rho d^2)$       \\
\textit{IGEL}                    & $\mathcal{O}(\delta_{\text{max}}^\alpha |V|)$   & $\mathcal{O}(\alpha \delta_{\text{max}} d)$     \\ \bottomrule
\end{tabular}
\label{tab:ComplexityComparison}
\caption*{\scriptsize \textsuperscript{} \textsuperscript{*}Struct2vec's authors describe its complexity in two terms. First, an $\mathcal{O}({|V|} \log |V|)$ preprocessing step to generate a structural meta-graph. Second, the structural embedding training process, equivalent to running DeepWalk over the meta-graph. We report the dominating time complexity of the preprocessing step.} 
\end{table}



==> Sections/introduction.tex <==
Graph structures are the natural way to represent arbitrary relationships in complex domains. Because of their generality, they can be applied to problems in which represented entities display rich interactions between each other. However, compactly capturing such interactions is a non-trivial task, often made unfeasible, for example, by the high-dimensionality and complexity of real-world networks.

Representation learning has been successfully applied to graphs, capturing useful interactions in compact ways~\cite{hamilton2017representation}. The learned representations can be used for downstream machine learning tasks, and have seen applications as varied as molecule generation for drug design~\cite{JMLR:v21:19-671}, content recommendation in social platforms~\cite{Ying-2018-PinSAGE}, or social network analysis~\cite{DBLP:journals/corr/PerozziAS14-deepwalk}.

A wide array of learning approaches have focused on local node features and interactions. \emph{Transductive} approaches require all nodes in the graph to be available at training time to learn a representation for each of them. Transductive methods can capture rich relationships within networks in a scalable manner. However, the resulting representations do not generalize to unseen nodes or edges, and require additional attention to deal with label permutations. 

In contrast, \emph{inductive} approaches~\cite{DBLP:journals/corr/HamiltonYL17-GraphSAGE} aim to compactly represent network interactions so that the specific identity of a node is irrelevant to its representation. Inductive representations are typically derived from attributes of nodes and edges within their neighbourhoods. In either case, inductive models tend to be more demanding than their transductive counterparts, particularly when entire graphs or node neighbourhoods ought to be sampled during training~\cite{DBLP:journals/corr/KipfW16-SemiSup-GCN}.  

In this paper, we introduce \textbf{IGEL} (\textbf{I}nductive \textbf{G}raph \textbf{E}mbeddings through \textbf{L}ocality Encoding), a novel inductive method for learning structural graph embeddings. IGEL aims to overcome the aforementioned issues in previous works by representing network structures explicitly, in the form of neighbourhood structure dictionaries. Dense vector representations are then learned from the structural dictionaries, in either an unsupervised graph-dependent process or under full supervision for a target task. 

We organize the paper as follows: in  \autoref{sec:RelatedWork}, we discuss the main lines of ongoing research in the state-of-the-art. Afterwards, we describe our model in \autoref{sec:IGELOverview}. In \autoref{sec:Experiments} we further explain our model in practical terms and show our experimental results. We go on to discuss the scalability of the method in \autoref{sec:Scalability}. Finally, we discuss our results and note the limitations of our model, wrapping up our analysis in \autoref{sec:Conclusions}.


==> Sections/related_work.tex <==
In this section, we briefly review the contributions most related to our work, grouping them according to their setting and their associated limitations. We then describe IGEL in this context, and give an introduction to how the method serves as a solution to existing problems. For a more comprehensive review of graph embedding techniques at large, we refer the reader to existing surveys~\cite{GOYAL201878, DBLP:journals/corr/abs-1901-00596}. 

\subsection{Unattributed Graph Embeddings}

First approaches to learning graph representations were applicable in unattributed settings as exemplified by models such as DeepWalk \cite{DBLP:journals/corr/PerozziAS14-deepwalk}. DeepWalk reduces the problem of learning compact node representations to the task of training a word2vec \cite{DBLP:journals/corr/abs-1301-3781} skip-gram language model over sequences of node labels sampled with random walks generated from a graph. Later, node2vec \cite{DBLP:journals/corr/GroverL16-node2vec} further extended this idea by introducing additional parameters to control the locality of the random walks, and thus, the properties of the learned latent spaces. 

An alternative transductive approach, LINE \cite{DBLP:journals/corr/TangQWZYM15-LINE}, tackled the problem by learning representations on the basis of structure. LINE minimizes the KL-divergence between the probability distribution of distinguishing adjacent nodes and between nodes with similar edges out of learned representations. The use of pairwise similarity measures has been further explored more recently by VERSE~\cite{DBLP:journals/corr/abs-1803-04742-VERSE}. VERSE tailors similarity measures such as personalized PageRank or SymRank into the loss function, aiming to capture explicit properties from underlying network relationships in contrast to context-based language models.

\textbf{Problem A.} The aforementioned methods are scalable and showed remarkable results in representing graphs in varied settings. However, they are limited by their nature as transductive approaches, namely, that the representations do not generalize to unseen nodes, edges or graphs.

\subsection{Convolutional Graph Networks}

More recently, research has focused on methods that learn inductive graph representations. Inductive representations are attractive as they can be applied on either transductive or inductive settings, so long as the same attributes are available on seen and unseen problem instances. Early models, such as Planetoid~\cite{DBLP:journals/corr/YangCS16-Planetoid} derived their representations from an embedding layer in a neural network whose input included node attributes, to perform semi-supervised training on classification tasks. 

However, a key component of graph data is that connected nodes can hold profound relationships between each other. Capturing those relationships can be a complex task, and much work has been devoted to it, particularly on works with Graph Convolutional Networks (GCNs) \cite{DBLP:journals/corr/NiepertAK16-GCN}. GCNs aggregate features from local neighbourhoods and the attributes of their nodes in order to generate a new feature representation for a given node. Because of this, they are ideal to capture the interactions between nodes and their neighbours. As such, GCNs have been successfully applied tasks such as semi-supervised learning
~\cite{DBLP:journals/corr/KipfW16-SemiSup-GCN} or node classification \cite{velikovi2017graph-GAT}. However, training GCNs when working on massive graphs is a challenge. 

In this direction, some work has focused on sampling the graph during training, as proposed by LGCL~\cite{DBLP:journals/corr/abs-1808-03965-LGCL} and GraphSAGE~\cite{DBLP:journals/corr/HamiltonYL17-GraphSAGE}. LGCL starts from a set nodes selected randomly and adds nodes incrementally by sampling according to a BFS strategy, until a budget of nodes is reached. %BFS to sample larger parts of the graph. % samples parts of large graphs into smaller ones by selecting a number of random nodes and then adding new nodes to the sub-graph as they are found through BFS.
Similarly, GraphSAGE represents a node by sampling a fixed number of neighbours at each distance from the node. This sampling approach bounds computational cost to a constant factor, trading off computational cost for predictive performance.

Based on this idea, methods such as PinSAGE~\cite{Ying-2018-PinSAGE} have shown promising results by building inductive models that can cope with web-scale problems by adapting sampling-based models to distributed environments.

\textbf{Problem B.} GCN models are applied in the presence of attributed data on nodes or edges. Applying them to unattributed networks is not straightforward, and it is not clear how the representations capture structural aspects or in tasks that require learning from node-to-node relationships. 

\subsection{Structural Representations}

To this end, models such as struct2vec~\cite{DBLP:journals/corr/FigueiredoRS17-struct2vec}, have been proposed to deal with graph substructures directly. Particularly, struct2vec tackles the issue by learning skip-gram representations on a constructed meta-graph that connects structurally-similar nodes within a threshold. 

\textbf{Problem C.} Constructing a meta-graph is a computationally costly process, as it relies on computing a pair-wise structural similarity measure across all nodes. Struct2vec proposes a series of optimizations to reduce the would-be quadratic computational cost, however, the learned representations remain label-dependent and, thus, they are affected by the aforementioned limitations of transductive approaches.

\subsection{Our Contribution in Context}

In this work, we tackle some of the problems we described about existing graph representation methods, namely:
\begin{enumerate}
    \item[\textbf{Problem A}] \emph{The difficulty in translating transductive network embeddings such as DeepWalk or node2vec to unseen graphs from the same domain}. Rather than working with individual nodes, we learn embeddings of graph structures, which capture more general properties of the graph.
    \item[\textbf{Problem B}] \emph{Graph Convolutional Networks on unattributed graphs leverage node and edge attributes}. We propose an inductive yet unattributed representation learning method. The resulting embeddings can serve potentially as additional input features to deep neural networks or graph convolutions.
    \item[\textbf{Problem C}] \emph{The scalability problems of existing structural embedding methods}. Methods such as struct2vec~\cite{DBLP:journals/corr/FigueiredoRS17-struct2vec} require to compute a similarity multilayer graph, which is expensive. We propose a similar structural representation, but avoid computing meta-graph structures by borrowing random-walk sampling techniques to learn an inductive representation.
\end{enumerate}

In the next section, we detail how IGEL functions, relating the building blocks of the method with the problems we seek to solve.



==> Sections/scalability.tex <==
%Our last task is to analyse the scalability of the proposed method. First, we study IGEL under the lens of time and parameter complexity. This helps contextualize the method with respect to existing art, and we believe can act as a compass for future efforts. Them, we proceed to empirically evaluate our specific implementation of the method. 

\subsection{Complexity Analysis}\label{sec:Scalability}

%In this section we describe the complexity of IGEL as it relates to other methods. In particular, we describe the time complexity of methods in terms of optimization steps during training. That is, a complexity $\mathcal{O}(|V|)$ implies that the training process is roughly dependent on the number of nodes in the graph. Furthermore, we detail the parameter complexity of each of the models, that is, the number of parameters given the hyper-parameters that affect them.

%\begin{table}[!h]
%\centering
%\caption{A comparison of graph representation methods in terms of their average parameter and time complexities. $\alpha$ stands for encoding distance in the case of IGEL or convolutional depth in GCNs, $r$ is the sampling factor for sampling GCNs, $\gamma$ is the average degree and $d$ is either the size of the embedding vectors or the number of features, as it applies in each method. $m$, as before, stands for maximum degree.}
%\begin{tabular}{@{}lrr@{}}
%\toprule
%\textbf{Name}               & \textbf{Time Complexity} & \textbf{Parameter Complexity} \\ \midrule
%\textit{DeepWalk, node2vec} & $\mathcal{O}(|V|)$       & $\mathcal{O}(|V|d)$       \\
%\textit{struct2vec}\textsuperscript{*} & $\mathcal{O}(|V|)$   & $\mathcal{O}(|V|d)$       \\
%\textit{GCN}                & $\mathcal{O}(\alpha |V| |E|)$ & $\mathcal{O}(\alpha d^2)$       \\
%\textit{GraphSAGE, LGCL}    & $\mathcal{O}(r^\alpha |V|)$   & $\mathcal{O}(\alpha d^2)$       \\
%\textit{IGEL}               & $\mathcal{O}(\gamma^\alpha |V|)$   & $\mathcal{O}(\alpha m d)$        \\ \bottomrule
%\end{tabular}
%\caption*{\scriptsize \textsuperscript{*}Struct2vec creates a pair-wise meta-graph as a preprocessing step. The meta-graph involves computing structural similarities, with an overall cost $\mathcal{O}({|V|} \log |V|)$.}
%\label{tab:ComplexityComparison}
%\end{table}

%\subsection{Experimental Evaluation}

We finish this experimental evaluation with an empirical analysis of the computational complexity of IGEL. For that, we evaluate our implementation in the unsupervised setting using synthetic data generated according to the Erdös-Renyi model. We control for three aspects that condition the runtime of the algorithm: the number of nodes $|V|$, the encoding distance $\alpha$, and the average degree per node. 

The training process is then performed with a realistic parameter configuration for encoding distances $\alpha= 1,2,3$. For each training configuration, we execute five independent experiments. Each run is performed on a Slurm-based cluster requesting 48 cpu cores and 200GB of memory on each setting. We record the overall training times, and analyze the run-time as a function of the size of the graph and the average degree.


%We test with an increase the number of nodes, iterating from $256$ to $16 384$ total nodes in the graph by factors of $4$, and generate edges to study networks with varying average degrees ranging from 4 to 16. 

%To experimentally evaluate the scalability of IGEL, we train unsupervised  models controlling the three key aspects impacting the performance of the method: number of nodes, average degree per node and encoding distance. To produce our training set, we generate random graphs according to the Erdös-Renyi model. We exponentially increase the number of nodes, iterating from $256$ to $16 384$ total nodes in the graph by factors of 4, and generate edges to study networks with varying average degrees ranging from 4 to 16. 

\begin{figure}[!h]
    \centering
    \begin{subfigure}{0.49\linewidth}
        \centering
         \includegraphics[width=\linewidth]{Scalability/ScalabilityNodesRuntime.pdf}
        %\caption{Average run times for graphs of different sizes with an average degree of 8. }
        \label{fig:ScalabilityResultsNode}
    \end{subfigure}
    \begin{subfigure}{0.49\linewidth}
        \centering
        \includegraphics[width=\linewidth]{Scalability/ScalabilityEdgesRuntime.pdf}
        %\caption{Average run times with a 4096-node graph on different values of average degree.}
    \end{subfigure}
    \caption{Scalability analysis.
    \textbf{(left)} Log-log plot showing the average runtime as a function of the graph size $|V|$ for different values of encoding distance $\alpha$ with fixed average degree of 8.
    \textbf{(right)} Average runtime as a function of the average degree for different values of $\alpha$ with fixed size of $|V|=4,096$.}
    %We study the impact of larger graphs with more nodes (left) and denser graphs with higher average degrees (right).}
    \label{fig:ScalabilityResults}
\end{figure}

\autoref{fig:ScalabilityResults} (a) shows the run-time as a function of the number of nodes $|V|$ for different values of the encoding distance $\alpha$, keeping the average degree fixed.
We observe that $\alpha$ does not significantly affect the cost in this setting. Furthermore all curves show an approximate linear scaling for $|V|\geq 1,024$ (note the log-scale in both axes), showing that IGEL can be applied to large-scale graphs in this regime.

%number of nodes, assuming a fixed average degree. We find that the encoding distance does not imply large performance costs, as our implementation caches the sparse structural vectors. However, higher values of $\alpha$ imply larger memory usage, and we find our executions run out of memory when $\alpha = 3$, on graphs with $16 384$ nodes where the average degree is higher than 8. We believe our cache implementation can be easily improved by representing the cache as contiguous in-memory arrays rather than python lists, and consider this an avenue of future work to ensure that the method can scale to denser and larger graphs.

We also analyze the influence of the average degree for different values of $\alpha$ in~\autoref{fig:ScalabilityResults} (b).
In this case, for $\alpha = 1$, we observe an almost constant
runtime as a function of the average degree, suggesting that the direct structural features can be feasibly applied to denser graphs. On the other hand, the runtime grows linearly with the average degree for values of $\alpha>2$, which is an actual limitation of IGEL in large-scale, dense networks.
\footnote{Our Python code, available at \url{https://github.com/nur-ag/IGEL}, can be admittedly improved using a sparse implementation of the structural representations, or a more memory-efficient programming language.}

%Finally, we make all of our code, training configurations and experimental results available \footnote{} to encourage parallel research, allow the community to replicate our results and provide a basis for future work.


%notice similar performance across varying values of encoding distances, hinting that direct structural features can be feasibly applied to potentially denser graphs. We believe this result is particularly interesting as it is a lower encoding distance that produces significantly better results for multi-label classification in the previous section. 
%This is to be expected, as in any case the sparse structural vector will grow larger and more densely populated. However, when $\alpha = 1$, we notice similar performance across varying values of encoding distances, hinting that direct structural features can be feasibly applied to potentially denser graphs. We believe this result is particularly interesting as it is a lower encoding distance that produces significantly better results for multi-label classification in the previous section. 

%the cpu-time as a function of the number of nodes $|V|$ of the graph, for a fixed value of eight for the average degree.
%We observe that the encoding distance $\alpha$ does not significantly change the cost in this setting, and that all curves show an approximate linearly scaling for $|V|\geq>1,024$.
%In the same direction, we notice that IGEL shows distinct performance curves iterating through graphs with different average degrees and while using higher encoding distances. This is to be expected, as in any case the sparse structural vector will grow larger and more densely populated. However, when $\alpha = 1$, we notice similar performance across varying values of encoding distances, hinting that direct structural features can be feasibly applied to potentially denser graphs. We believe this result is particularly interesting as it is a lower encoding distance that produces significantly better results for multi-label classification in the previous section. 

%Our scalability analysis highlights limitations of our implementation and potential avenues for future work in relation with \autoref{tab:ComplexityComparison}. Asymptotically, we expect a constant slope in \autoref{fig:ScalabilityResultsNode}, which experimentally we observe for larger graphs with $|V| > 1 024$. In a broader sense,

Overall, these results show that IGEL is a scalable method for values of $\alpha = 1,2$. We believe that ideas from sampling-based GCN literature can be extended to purely structural methods like IGEL to allow for the encoding and learning of very distant structural features.
